Commutative and non-commutative bialgebras of quasi-posets and applications to Ehrhart polynomials

To any poset or quasi-poset is attached a lattice polytope, whose Ehrhart polynomial we study from a Hopf-algebraic point of view. We use for this two interacting bialgebras on quasi-posets. The Ehrhart polynomial defines a Hopf algebra morphism taking its values in Q[X], we deduce from the interacting bialgebras an algebraic proof of the duality principle, a generalization and a new proof of a result on B-series due to Whright and Zhao, using a monoid of characters on quasi-posets, and a generalization of Faulhaber's formula. We also give non-commutative versions of these results: polynomials are replaced by packed words. We obtain in particular a non-commutative duality principle.

==> arbresbinaires.tex <==
%Arbres binaires

\newcommand{\bun}{
\begin{picture}(5,5)(-2,0)
\put(0,0){\line(0,0){5}}
\end{picture}}

\newcommand{\bdeux}{
\begin{picture}(10,15)(-5,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\end{picture}}

\newcommand{\btroisun}{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\end{picture}}
\newcommand{\btroisdeux}{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\end{picture}}

\newcommand{\bquatreun}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-9.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatredeux}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-6.3,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatretrois}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(-3.5,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrequatre}{
\begin{picture}(15,25)(-7,0)
\put(-3.5,4.1){$\vee$}
\put(0,0){\line(0,1){5}}
\put(-0.7,10.7){$\vee$}
\put(2.1,17.3){$\vee$}
\end{picture}}
\newcommand{\bquatrecinq}{
\begin{picture}(15,20)(-7,0)
\put(0,0){\line(0,1){5}}
\put(0,5){\line(2,1){10}}
\put(0,5){\line(-2,1){10}}
\put(-3,6.5){\line(0,1){5}}
\put(3,6.5){\line(0,1){5}}
\end{picture}}

%Arbres binaires décorés

\newcommand{\bddeux}[1]{
\begin{picture}(25,22)(-12,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){10}}
\put(-9,7){\tiny #1}
\end{picture}}

\newcommand{\bdtroisun}[2]{
\begin{picture}(25,22)(-14,5)
\drawline(0,0)(0,7)(-14,21)
\drawline(0,7)(7,14)
\drawline(-7,14)(0,21)
\put(-7,4){\tiny #1}
\put(-14,11){\tiny #2}
\end{picture}}

\newcommand{\bdtroisdeux}[2]{
\begin{picture}(25,22)(-10,5)
\drawline(0,0)(0,7)(14,21)
\drawline(0,7)(-7,14)
\drawline(7,14)(0,21)
\put(2,4){\tiny #1}
\put(9,11){\tiny #2}
\end{picture}}

\newcommand{\bddtroisun}[5]{
\begin{picture}(30,40)(-20,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){10}}
\put(0,10){\line(-1,1){20}}
\put(-10,20){\line(1,1){10}}
\put(-9,7){\tiny #1}
\put(-19,17){\tiny #2}
\put(-21,32){\tiny #3}
\put(-1,32){\tiny #4}
\put(9,22){\tiny #5}
\end{picture}}
\newcommand{\bddtroisdeux}[5]{
\begin{picture}(30,40)(-10,0)
\put(0,0){\line(0,0){10}}
\put(0,10){\line(1,1){20}}
\put(0,10){\line(-1,1){10}}
\put(10,20){\line(-1,1){10}}
\put(3,7){\tiny #1}
\put(13,17){\tiny #2}
\put(-11,22){\tiny #3}
\put(-1,32){\tiny #4}
\put(19,32){\tiny #5}
\end{picture}}

